State Space Models are Strong Text Rerankers

Transformers dominate NLP and IR; but their inference inefficiencies and challenges in extrapolating to longer contexts have sparked interest in alternative model architectures. Among these, state space models (SSMs) like Mamba offer promising advantages, particularly $O(1)$ time complexity in inference. Despite their potential, SSMs' effectiveness at text reranking -- a task requiring fine-grained query-document interaction and long-context understanding -- remains underexplored. This study benchmarks SSM-based architectures (specifically, Mamba-1 and Mamba-2) against transformer-based models across various scales, architectures, and pre-training objectives, focusing on performance and efficiency in text reranking tasks. We find that (1) Mamba architectures achieve competitive text ranking performance, comparable to transformer-based models of similar size; (2) they are less efficient in training and inference compared to transformers with flash attention; and (3) Mamba-2 outperforms Mamba-1 in both performance and efficiency. These results underscore the potential of state space models as a transformer alternative and highlight areas for improvement in future IR applications.

==> figures/inference_profiling-125m.tex <==
\begin{figure*}
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/opt-125m.png}
        \caption{OPT-125M}
        \label{fig:profiling-opt-125m}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/opt-125m-flashattn.png}
        \caption{OPT-125M w/ Flash-Attn}
        \label{fig:profiling-opt-125m-flashattn}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mamba1-130m.png}
        \caption{Mamba-1-130M}
        \label{fig:profiling-mamba1-130m}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mamba2-130m.png}
        \caption{Mamba-2-130M}
        \label{fig:profiling-mamba2-130m}
    \end{subfigure}

\caption{
Inference profiling results for OPT-125M vs Mamba models of similar size.
}
\label{fig:profiling_appendix}
\vspace{-10pt}
\end{figure*}

==> tables/train_throughput.tex <==
\begin{table}[t!]
\vspace{0pt}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrr}
\toprule
\begin{tabular}[c]{@{}l@{}l} Model \\ \, \\ \end{tabular}
& \begin{tabular}[c]{@{}l@{}l} BZ \\ \, \\ \end{tabular}
& \begin{tabular}[c]{@{}l@{}l} Tokens per \\ second ($\uparrow$) \\ \end{tabular}
& \begin{tabular}[c]{@{}l@{}l} Rel. \\ Throughput ($\uparrow$) \\ \end{tabular} \\
\midrule
\multirow{4}{*}{BERT-large} & 1  & 11949      & 1x              \\
                            & 2  & 13292      & 1.12x           \\
                            & 4  & 14592      & 1.22x           \\
                            & 8  & OOM        & -               \\ 
\hline
\multirow{4}{*}{BART-large} & 1  & 15988      & 1.34x              \\
                            & 2  & 20604      & 1.72x           \\
                            & 4  & 24403      & 2.04x           \\
                            & 8  & OOM        & -               \\
\hline
\multirow{4}{*}{OPT-350m} & 1  & 20317      & 1.70x              \\
                            & 2  & 22624      & 1.89x           \\
                            & 4  & 25133      & 2.10x           \\
                            & 8  & 26193        & 2.19x               \\
\hline
\multirow{4}{*}{Mamba1-370m} & 1  & 9068      & 0.76x              \\
                            & 2  & 10000      & 0.84x           \\
                            & 4  & 10384      & 0.87x           \\
                            & 8  & OOM        & -               \\
\hline
\multirow{4}{*}{Mamba2-370m} & 1  & 10600      & 0.89x              \\
                            & 2  & 13761      & 1.15x           \\
                            & 4  & 16501      & 1.38x           \\
                            & 8  & 17634        & 1.48x               \\
\bottomrule
\end{tabular}
}
\caption{Train throughput of models$\approx$330M, OPT model is trained with FlashAttention-2. BZ denotes batch size and OOM denotes out of memory.}
\label{tab:throughput}
\end{table}
